Latent Transformations via NeuralODEs for GAN-based Image Editing

Recent advances in high-fidelity semantic image editing heavily rely on the presumably disentangled latent spaces of the state-of-the-art generative models, such as StyleGAN. Specifically, recent works show that it is possible to achieve decent controllability of attributes in face images via linear shifts along with latent directions. Several recent methods address the discovery of such directions, implicitly assuming that the state-of-the-art GANs learn the latent spaces with inherently linearly separable attribute distributions and semantic vector arithmetic properties. In our work, we show that nonlinear latent code manipulations realized as flows of a trainable Neural ODE are beneficial for many practical non-face image domains with more complex non-textured factors of variation. In particular, we investigate a large number of datasets with known attributes and demonstrate that certain attribute manipulations are challenging to obtain with linear shifts only.

==> tables/encoder.tex <==
\begin{table*}[htb!]
	\centering
		\begin{tabular}{l}
			\toprule
			ReLU \\ 
			FC \texttt{n\_channel} $\times$ \texttt{f\_size} \\
			ReLU \\ 
			$\{$FC \texttt{f\_size} $\times$ $\mathcal{S}_i \}_{i=1}^{N}$ \\
			\bottomrule
		\end{tabular}
	\caption{Multiclass classification module used for our encoders. \texttt{n\_channel} is $1024$ for the simple convolutional encoder and $512$ for the ResNet18 backbones. \texttt{f\_size} is $512$ for all the datasets except \emph{MPI3D} where it is $256$. $\mathcal{S}_i$ denotes the cardinality of the $i$-th attribute.}
	\label{tab:encoder_architecture}
\end{table*}
